Cross-Utterance Conditioned VAE for Speech Generation

Speech synthesis systems powered by neural networks hold promise for multimedia production, but frequently face issues with producing expressive speech and seamless editing. In response, we present the Cross-Utterance Conditioned Variational Autoencoder speech synthesis (CUC-VAE S2) framework to enhance prosody and ensure natural speech generation. This framework leverages the powerful representational capabilities of pre-trained language models and the re-expression abilities of variational autoencoders (VAEs). The core component of the CUC-VAE S2 framework is the cross-utterance CVAE, which extracts acoustic, speaker, and textual features from surrounding sentences to generate context-sensitive prosodic features, more accurately emulating human prosody generation. We further propose two practical algorithms tailored for distinct speech synthesis applications: CUC-VAE TTS for text-to-speech and CUC-VAE SE for speech editing. The CUC-VAE TTS is a direct application of the framework, designed to generate audio with contextual prosody derived from surrounding texts. On the other hand, the CUC-VAE SE algorithm leverages real mel spectrogram sampling conditioned on contextual information, producing audio that closely mirrors real sound and thereby facilitating flexible speech editing based on text such as deletion, insertion, and replacement. Experimental results on the LibriTTS datasets demonstrate that our proposed models significantly enhance speech synthesis and editing, producing more natural and expressive speech.

==> bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/liyang.jpg}}]{Yang Li} is a PhD candidate in Computer Science at the University of Manchester. His research interests include multi-agent systems, human-AI/Robot collaboration, and application of AI. Yang received a degree of master from the University of Chinese Academy of Sciences and a degree of bachelor from the Dalian University of Technology. Yang’s scholarly contributions include publications in prestigious conferences and journals, including ICML, ICLR, ACL, TMLR, TMC, TWC, and so on. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yucheng.jpg}}]
{Cheng Yu} received the Bachelor’s degree in Computer Science and Technology from ShanghaiTech University, Shanghai, China, in 2021, and the Master’s degree in the same field from ShanghaiTech University in 2024.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/brian.jpg}}]{Guangzhi Sun} is a research associate at the Machine Intelligence Lab, University of Cambridge. His research interest lies in controllable and reliable multi-modal conversational AI with large language models. He completed his PhD at the Department of Engineering, University of Cambridge under the supervision of Prof. Phil Woodland and advised by Prof. Mark Gales on contextual knowledge integration in end-to-end neural-based conversational AI systems. He held a research internship at Google Brain with Dr Yu Zhang in 2019 and ByteDance with Dr Wei Li in 2023. He received by B. A and M.Eng degree in 2019 at Trinity College, University of Cambridge. He was awarded the Best Student Paper in interspeech 2022.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/weiqin.jpg}}] {Weiqin~Zu}, Student Member, IEEE, received the B.S. degree in computer science and technology from ShanghaiTech University, Shanghai, China,in 2022. He is currently pursuing the master's degree with the School of Information Science and Technology, ShanghaiTech University, Shanghai, China. His research interests include multi-agent systems, human-robot interaction, and navigation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/Zheng_Tian.jpg}}] {Zheng Tian} is a machine learning researcher and an assistant professor at ShanghaiTech University. He studies Reinforcement Learning, Multi-Agent System and relevant applications in art and design. He has published several paper at top conferences, along with the best system paper award at CoRL 2020. He completed his Ph.D. degree, M.SC. degree and Bachelor degree at University College London.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/Ying_Wen.jpg}}]{Ying Wen} 
is a tenure-track tenure-track associate professor in School of Artificial Intelligence and John Hopcroft Center, Shanghai Jiao Tong University.. His research interests include machine learning, multi-agent systems and human-centered interactive systems etc. He has published over 40 research papers about machine learning on top-tier international conferences (ICML, NeurIPS,  ICLR, IJCAI, and AAMAS). He was granted Best Paper Award in AAMAS 2021 Blue Sky Track and the Best System Paper Award in CoRL 2020.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/weipan.jpg}}]{Wei Pan}is an Associate Professor in Machine Learning at the Department of Computer Science and a member of Centre for AI Fundamentals and Centre for Robotics and AI, The University of Manchester, UK. Before that, he was an Assistant Professor in Robot Dynamics at the Department of Cognitive Robotics and co-director of Delft SELF AI Lab, TU Delft, Netherlands, and a Project Leader at DJI, China. He is an Area Chair or Associate Editor of IEEE RAL, ACM TOPML, CoRL, L4DC, ICRA, IROS. He has a broad interest in robot control using Bayesian machine learning and the principles of dynamic control.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/chaozhang.jpg}}] {Chao Zhang}
     received his BE and MSc degrees in 2009 and 2012 from the Department of Computer Science and Technology, Tsinghua University, and his PhD in 2017 from the Cambridge University Engineering Department (CUED). He is an Assistant Professor at the Department of Electronic Engineering, Tsinghua University, and an Honorary Associate Professor at the Faculty of Brain Sciences, UCL. Before that, he was a Senior Research Scientist at Google, a Research Associate at CUED, and an advisor and speech team co-leader of JD.com. His research interests include spoken language processing, machine learning, and cognitive neuroscience. He has published 100 peer-reviewed speech and language processing papers and received multiple awards for best student papers from ICASSP, Interspeech, ASRU, and SLT.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/Jun_Wang.jpg}}] 
{Jun Wang} is Professor at the Computer Science Department, University College London. Prof. Jun Wang's main research interests are in the areas of AI and intelligent systems, covering (multiagent) reinforcement learning, deep generative models, and their diverse applications on information retrieval, recommender systems and personalization, data mining, smart cities, bot planning, and computational advertising. His team won the first global real-time bidding algorithm contest with 80+ participants worldwide. Jun has published over 200 research papers and is a winner of multiple Best Paper awards. He was a recipient of the Beyond Search --- Semantic Computing and Internet Economics award by Microsoft Research and also received Yahoo! FREP Faculty award. He has served as an Area Chair in ACM CIKM and ACM SIGIR. 
\end{IEEEbiography}


 % \vspace{-10mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/Yang_Yang.jpg}}] {Yang~Yang}, IEEE Fellow, is a Professor with the IoT Thrust, the Director of Research Center for the Digital World with Intelligent Things (DOIT), and the Associate Vice-President for Teaching and Learning at The Hong Kong University of Science and Technology (Guangzhou), China. He is also an adjunct professor with the Department of Broadband Communication at Peng Cheng Laboratory, the Chief Scientist of IoT at Terminus Group, and a Senior Consultant for Shenzhen Smart City Technology Development Group, China. Before joining HKUST (GZ), he has held faculty positions at the Chinese University of Hong Kong, Brunel University, U.K., University College London (UCL), U.K., CAS-SIMIT, and ShanghaiTech University, China. 
Yang's research interests include multi-tier computing networks, 5G/6G systems, AIoT technologies, intelligent services and applications, and advanced wireless testbeds. He has published more than 300 papers and filed more than 120 technical patents in these research areas. He has been the Chair of the Steering Committee of Asia-Pacific Conference on Communications (APCC) from 2019 to 2021. Currently, he is serving the IEEE Communications Society as the Chair for 5G Industry Community and Chair for Asia Region at Fog/Edge Industry Community. 

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/Fanglei_Sun.jpg}}] {Fanglei Sun} is currently an associate professor with the Department of Computer Science and Engineering at the University of Shanghai for Science and Technology. Her current research interests include machine learning, multi-agent systems, and intelligent design for communication systems. She has published over 40 papers in top-tier international journals and conferences, including TWC, TMC, IEEE IoT, TVT, ACL, ICRA, NeurIPS, ICLR, IJCAI, Globecom, and ICC. Additionally, she has filed over 50 Chinese and international patents in her focused research areas.
\end{IEEEbiography}
